Learning passive policies with virtual energy tanks in robotics

Within a robotic context, we merge the techniques of passivity-based control (PBC) and reinforcement learning (RL) with the goal of eliminating some of their reciprocal weaknesses, as well as inducing novel promising features in the resulting framework. We frame our contribution in a scenario where PBC is implemented by means of virtual energy tanks, a control technique developed to achieve closed-loop passivity for any arbitrary control input. Albeit the latter result is heavily used, we discuss why its practical application at its current stage remains rather limited, which makes contact with the highly debated claim that passivity-based techniques are associated with a loss of performance. The use of RL allows us to learn a control policy that can be passivized using the energy tank architecture, combining the versatility of learning approaches and the system theoretic properties which can be inferred due to the energy tanks. Simulations show the validity of the approach, as well as novel interesting research directions in energy-aware robotics.

==> introduction.tex <==
\section{Introduction}

Robotics is increasingly focusing on the development of control frameworks allowing the transition from industrial cages to unstructured environments. This transition carries the ambitious objective of stable and safe execution of complex tasks where robots coexist with other robots or possibly humans. The practical impossibility of careful dynamic modeling of the environment along those tasks makes the stability objective even more challenging, and model-based approaches poorly suitable.

Passive controllers have been presented as a feasible solution to tackle this problem as the stability of the closed-loop system is in principle independent on the external environmental interaction \cite{Stramigioli2015Energy-AwareRobotics,vanderSchaftL2}. Passive systems route physical energy rather than producing it, which is the ultimate reason why stability proofs (using energy functions as Lyapunov candidates) are conveniently assessed in this framework \cite{Duindam2009ModelingSystems,Ortega2004InterconnectionSurvey}. A powerful technique allowing the passivization of any control action is represented by \textit{virtual energy tanks} \cite{Califano2022OnSystems,Secchi2006PositionTelemanipulation,Duindam2004Port-basedSystems}. These are able to store information about physical energy flows undergoing the system, and introduce at a control level the scalar information representing the energy budget for the controlled robot. A conditional check on this budget with proper passive reaction strategies in case of depletion of the latter is what guarantees closed-loop passivity. The main drawback of passivity-based control methods (comprising those involving energy tanks) is the lack of optimization over a task performance metric along the design of the controller \cite{7384497}. This fact led to the claim that passivity-based control methods are associated with a loss of performance, which becomes more severe as the complexity of tasks increases.

On the other side of the control theoretic spectrum, recent advancements in the machine learning community are leading to robots with an outstanding awareness of complex environments and tasks. The intelligence encoded in the control policies, normally optimized by means of performance-based metrics, reflects complex high-level decision-making strategies which are learned thanks to the availability of huge datasets \cite{Zeng2018, Singh2019, Zhu2020}. The drawback of these families of approaches is the difficulty in guaranteeing system theoretic properties such as passivity and stability for the controlled system \cite{Busoniu2018ReinforcementApproximators}. 

In this work we merge the passivity-based control (PBC) design involving energy tanks and reinforcement learning framework (RL), combining system theoretic properties of the closed-loop system induced by the ultimately passive design, and high-performance achievement peculiar of the RL framework.
This procedure presented both in inference and in training, allows meaningful scale PBC to tasks requiring the learning of complex control policies.

 
\subsubsection*{Related work}
We recognize related work casting the energy tank algorithm (seen as a task-agnostic passivization tool) into a framework using task-based information for performance augmentation of the underlying passive system. In \cite{Shahriari2018Valve-basedObjectives} the authors introduce the so-called \textit{valve-based energy tanks} (also used in e.g., \cite{Benzi2022AdaptiveEstimation}), in which extra parameters are introduced on the energy tanks in order to embed control objectives in the design, beyond achieving passivity. Task specifications are translated into tank design rules by controlling the power flows undergoing the system. The idea of using a reference power trajectory in combination with energy tanks is present also in \cite{Shahriari2020PowerTanks,califano22}, where task-based specifications are used to tune the tank parameters. These works present very stiff task specifications and badly scale to complex tasks in which high-level policies need to be learned. 
A family of methods using energy tanks and sharing a similar motivation of this work is \cite{benzi22,Capelli2022PassivityEnergy}, where an explicit optimization problem is introduced to find the closest passive approximation of a given control action. The idea is to exploit the versatility of energy tank architecture to perform an optimization that can be generalized and scaled for different tasks and whose outcome is a passively controlled system. An important difference between this work and the cited ones (beyond the specific technique to solve the optimization) is that in \cite{benzi22,Capelli2022PassivityEnergy} the desired control action is already given, and the optimization aims at finding the closest passive approximation to it, imposed by a non-depletion constraint of the tank. We will comment on the difference between the approaches, which involves the degree of freedom represented by the initial state in the tank.

The paper is organized as follows. In Sec. \ref{sec:background} a throughout explanation of the PBC problem in robotics and its achievement using energy tanks is reviewed, followed by a discussion regarding the limitations of the methodology. In Sec. \ref{sec:framework} the proposed scheme is presented, and validated in Sec. \ref{sec:simulations} by means of different simulations. Conclusions and future works are sketched in Sec. \ref{sec:Conclusion}.


==> simulation.tex <==
 
\subsection{Experiment 1}
To show the effects of the passivization in inference an external force is applied to the system in order to make it to consume more energy. For this experiment we consider the \texttt{DoorOpening} environment. As visible in Figure \ref{fig:inferencewind} the trained and tested without the passivization under the external force (pushing the robot toward the door) $\phi_{\infty|\infty,w}$ has can use an unbounded amount of energy, while the same agent under the effect of the same force but wrapped by the passivization framework in inference $\phi_{\infty|e^*,w}$ can consume an amount of energy with is limited by the initialization of the energy tank. Figure \ref{fig:inferencewind} also shows the average energy of the agent under normal conditions (without the external force) and without passivization $\phi_{\infty|\infty,w}$. In this case, the energy used is not limited but it is used to find the task energy.
 
%all the 3 environments \textit{Pendulum}, \textit{HalfCheetah} and \textit{DoorOpening}. For each environment an agent $\phi_\infty$ has been trained. 

%In particualr, we used the pretrained model available online \footnote{https://github.com/ARISE-Initiative/robosuite-benchmark} for \textit{RobotDoorOpening}, while for \textit{HalfCheetah} and \textit{InvertedPendulum} we trained the agent using  the hyperparameters from \cite{rl-zoo3} 


\begin{figure}[t]
    \centering
     \includegraphics[ width=\columnwidth]{figures/plots/dooropening/pandadoor_inference_energy.pdf}
    \caption{Average energy spent in \texttt{DoorOpening} environment during an episode in inference.  $\phi_{\infty|\infty,w}$ represents the agent tested without passivization, $\phi_{\infty|\infty,w}$ represents the same agent under the effects of an external force, while $\phi_{\infty|e^*,w}$ is the agent wrapped by the passivization framework}
    \label{fig:inferencewind}
\end{figure}

% \begin{figure*}[t]
%     \centering
%     \subfloat[\texttt{DoorOpening}]{
%         \centering
%         \includegraphics[width=.6\columnwidth]{figures/plots/passive_inference/pandadoor_inference_energy.pdf}
%         \label{fig:infmin/train/return}
%     } \hfill 
%     \subfloat[\texttt{HalfCheetah}]{
%         \centering
%         \includegraphics[width=.6\columnwidth]{figures/missing.pdf}
%         \label{fig:infmin/train/return}
%     } \hfill 
%     \subfloat[ \texttt{Pendulum}]{
%         \centering
%         \includegraphics[width=.6\columnwidth]{figures/missing.pdf}
%         \label{fig:infmin/train/return}
%     } 
%     \caption{Total energy spent over the episode in inference
%     }
%     \label{fig:passive_inference_wind} 
% \end{figure*}
